Generalizable Pose Estimation Using Implicit Scene Representations

6-DoF pose estimation is an essential component of robotic manipulation pipelines. However, it usually suffers from a lack of generalization to new instances and object types. Most widely used methods learn to infer the object pose in a discriminative setup where the model filters useful information to infer the exact pose of the object. While such methods offer accurate poses, the model does not store enough information to generalize to new objects. In this work, we address the generalization capability of pose estimation using models that contain enough information about the object to render it in different poses. We follow the line of work that inverts neural renderers to infer the pose. We propose i-$\sigma$SRN to maximize the information flowing from the input pose to the rendered scene and invert them to infer the pose given an input image. Specifically, we extend Scene Representation Networks (SRNs) by incorporating a separate network for density estimation and introduce a new way of obtaining a weighted scene representation. We investigate several ways of initial pose estimates and losses for the neural renderer. Our final evaluation shows a significant improvement in inference performance and speed compared to existing approaches.

==> figures/experiments/car_convergence/car_convergence.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/car_convergence/input.png}
         \caption{target}
         \label{fig:car_conv_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/car_convergence/rgb_0.png}
         \caption{step 0}
         \label{fig:car_conv_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/car_convergence/rgb_100.png}
         \caption{step 100}
         \label{fig:car_conv_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/car_convergence/rgb_299.png}
         \caption{step 299}
         \label{fig:car_conv_d}
     \end{subfigure}
    \caption{\textbf{Converging to the target.} a) is the target image and b) to d) are snapshots to the solution with the lowest L1 loss.}
    \label{fig:car_convergence}
    \vspace{-0.5cm}
\end{figure}

==> figures/experiments/convergence_plots/A_2shot/A_2shot.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/A_2shot/input.png}
         \caption{target}
         \label{fig:conv_A_2shot_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/A_2shot/rgb_0.png}
         \caption{step 0}
         \label{fig:conv_A_2shot_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/A_2shot/rgb_100.png}
         \caption{step 100}
         \label{fig:conv_A_2shot_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/A_2shot/rgb_299.png}
         \caption{step 299}
         \label{fig:conv_A_2shot_d}
     \end{subfigure}
    \caption{\textbf{Converging to the target.} a) is the target image and b) to d) are snapshots to the solution with the lowest L1 loss.}
    \label{fig:convergence_A_2shot}
    \vspace{-0.5cm}
\end{figure}

==> figures/experiments/convergence_plots/B_2shot/b_2shot.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/input.png}
         \caption{target}
         \label{fig:conv_B_2shot_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/rgb_0.png}
         \caption{step 0}
         \label{fig:conv_B_2shot_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/rgb_100.png}
         \caption{step 100}
         \label{fig:conv_B_2shot_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/rgb_299.png}
         \caption{step 299}
         \label{fig:conv_B_2shot_d}
     \end{subfigure}
    \caption{\textbf{Converging to the target.} a) is the target image and b) to d) are snapshots to the solution with the lowest L1 loss.}
    \label{fig:convergence_B_2shot}
    \vspace{-0.5cm}
\end{figure}

==> figures/experiments/convergence_plots/D/D.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/input.png}
         \caption{target}
         \label{fig:conv_D_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/rgb_0.png}
         \caption{step 0}
         \label{fig:conv_D_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/rgb_100.png}
         \caption{step 100}
         \label{fig:conv_D_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/rgb_299.png}
         \caption{step 299}
         \label{fig:conv_D_d}
     \end{subfigure}
    \caption{\textbf{Converging to the target.} a) is the target image and b) to d) are snapshots to the solution with the lowest L1 loss.}
    \label{fig:convergence_D}
    \vspace{-0.5cm}
\end{figure}

==> figures/experiments/convergence_plots/E/E.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/E/input.png}
         \caption{target}
         \label{fig:conv_E_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/E/rgb_0.png}
         \caption{step 0}
         \label{fig:conv_E_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/E/rgb_100.png}
         \caption{step 100}
         \label{fig:conv_E_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/E/rgb_299.png}
         \caption{step 299}
         \label{fig:conv_E_d}
     \end{subfigure}
    \caption{\textbf{Converging to the target.} a) is the target image and b) to d) are snapshots to the solution with the lowest L1 loss.}
    \label{fig:convergence_E}
    \vspace{-0.5cm}
\end{figure}

==> figures/experiments/convergence_plots/all.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/A_2shot/input.png}
         \label{fig:conv_A_2shot_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/A_2shot/rgb_0.png}
         \label{fig:conv_A_2shot_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/A_2shot/rgb_100.png}
         \label{fig:conv_A_2shot_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/A_2shot/rgb_299.png}
         \label{fig:conv_A_2shot_d}
     \end{subfigure}
          \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/input.png}
         \label{fig:conv_B_2shot_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/rgb_0.png}
         \label{fig:conv_B_2shot_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/rgb_100.png}
         \label{fig:conv_B_2shot_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/rgb_299.png}
         \label{fig:conv_B_2shot_d}
     \end{subfigure}
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/input.png}
         \label{fig:conv_D_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/rgb_0.png}
         \label{fig:conv_D_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/rgb_100.png}
         \label{fig:conv_D_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/rgb_299.png}
         \label{fig:conv_D_d}
     \end{subfigure}
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/E/input.png}
         \caption{target}
         \label{fig:conv_E_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/E/rgb_0.png}
         \caption{step 0}
         \label{fig:conv_E_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/E/rgb_100.png}
         \caption{step 100}
         \label{fig:conv_E_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/E/rgb_299.png}
         \caption{step 299}
         \label{fig:conv_E_d}
     \end{subfigure}
    \caption{\textbf{Converging to the target.} a) is the target image and b) to d) are snapshots to the solution with the lowest L1 loss.}
    \label{fig:convergence_All}
    \vspace{-0.5cm}
\end{figure}

==> figures/experiments/convergence_plots/non_2shot_2shot.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/input.png}
         \caption{Target}
         \label{fig:conv_D_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/rgb_0.png}
         \caption{Step 0}
         \label{fig:conv_D_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/rgb_100.png}
         \caption{Step 100}
         \label{fig:conv_D_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/D/rgb_299.png}
         \caption{Step 299}
         \label{fig:conv_D_d}
     \end{subfigure}
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/input.png}
         \renewcommand{\thesubfigure}{a}%
         \caption{Target}
         \label{fig:conv_B_2shot_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/rgb_0.png}
         \renewcommand{\thesubfigure}{b}%
         \caption{Step 0}
         \label{fig:conv_B_2shot_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/rgb_100.png}
         \renewcommand{\thesubfigure}{c}%
         \caption{Step 100}
         \label{fig:conv_B_2shot_c}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/experiments/convergence_plots/B_2shot/rgb_299.png}
         \renewcommand{\thesubfigure}{d}%
         \caption{Step 299}
         \label{fig:conv_B_2shot_d}
     \end{subfigure}
    \caption{\textbf{Converging to the target.} a) is the target image and b) to d) are snapshots to the solution with the lowest L1 loss.}
    \label{fig:convergence_2shot}
    \vspace{-0.5cm}
\end{figure}

==> tables/eval_time.tex <==
\begin{table}[htbp]
\caption{Eval time per batch.}
\begin{center}
\begin{tabular}{lr}
\toprule
\textbf{Method}&\textbf{Time} \\
\midrule
\textbf{i-NeRF} &  \\
\textbf{i-$\sigma$SRN (ours)} &  \\
\bottomrule
\end{tabular}
\label{tab:eval_cars} 
\end{center}
\end{table}

==> tables/scores_assembly.tex <==
\begin{table}[htbp]
\caption{Pose estimation errors on the Assembly dataset.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc}
\toprule
\textbf{Method} & \textbf{Inference} &\multicolumn{2}{c}{\textbf{Pose Estimation errors}}\\
\cmidrule{3-4} 
 & &  \textbf{\textit{Rotation}}& \textbf{\textit{Translation}}  \\
\midrule
\textbf{i-NeRF} & single & 46.66 & 0.55 \\
\textbf{i-NeRF} & multiple (10) & 46.55 & 0.52 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (fixed, 24) & 3.59 & 0.01 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (neighbor, 4) &  2.36 & 0.01 \\
\bottomrule
\end{tabular}
}
\label{tab:pose-assembly}
\end{table}

==> tables/scores_cars.tex <==
\begin{table}[htbp]
\caption{Pose estimation errors on the Shapenet Cars dataset.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc}
\toprule
\textbf{Method} & \textbf{Inference} &\multicolumn{2}{c}{\textbf{Pose Estimation errors}}\\
\cmidrule{3-4} 
 & &  \textbf{\textit{Rotation}}& \textbf{\textit{Translation}} \\
\midrule
\textbf{i-NeRF} & single & 32.24 & 0.61 \\
\textbf{i-NeRF} & multiple (10) & 24.88 & 0.60 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (fixed, 24) & 2.60 & 0.02 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (neighbor, 4) & 1.38 & 0.02 \\
\bottomrule
\end{tabular}
}
\label{tab:pose-cars}
\end{table}

==> tables/scores_chairs.tex <==
\begin{table}[htbp]
\caption{Pose estimation errors on the Shapenet Chairs dataset.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc}
\toprule
\textbf{Method} & \textbf{Inference} &\multicolumn{2}{c}{\textbf{Pose Estimation errors}} \\
\cmidrule{3-4} 
 & &  \textbf{\textit{Rotation}}& \textbf{\textit{Translation}} \\
\midrule
\textbf{i-NeRF} & single & 17.30 & 0.94 \\
\textbf{i-NeRF} & multiple (10) & 16.87 & 0.91 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (fixed, 24) & 30.54 & 0.09 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (neighbor, 4) & 12.87 & 0.08 \\
\bottomrule
\end{tabular}
}
\label{tab:pose-chairs}
\end{table}

==> tables/scores_fewshot_assembly.tex <==
\begin{table}[htbp]
\caption{Few-Shot Pose estimation errors on the Assembly dataset.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc}
\toprule
\textbf{Method} & \textbf{Inference} &\multicolumn{2}{c}{\textbf{Pose Estimation errors}}\\
\cmidrule{3-4} 
 & &  \textbf{\textit{Rotation}}& \textbf{\textit{Translation}}  \\
\midrule
\textbf{i-NeRF} & 2-shot samples & 83.76 & 1.09 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (fixed, 24) & 63.69 & 0.1 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (neighbor, 4) &  32.48 & 0.09 \\
\bottomrule
\end{tabular}
}
\label{tab:few-shot-assembly}
\end{table}

==> tables/scores_fewshot_cars.tex <==
\begin{table}[htbp]
\caption{Few-Shot Pose estimation errors on the Shapenet Cars dataset.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc}
\toprule
\textbf{Method} & \textbf{Inference} &\multicolumn{2}{c}{\textbf{Pose Estimation errors}}\\
\cmidrule{3-4} 
 & &  \textbf{\textit{Rotation}}& \textbf{\textit{Translation}}  \\
\midrule
\textbf{i-NeRF} & 2-shot samples & 105.78 & 1.47 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (fixed, 24) & 38.37 & 0.13 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (neighbor, 4) &  14.59 & 0.12 \\
\bottomrule
\end{tabular}
}
\label{tab:few-shot-cars}
\end{table}

==> tables/scores_fewshot_chairs.tex <==
\begin{table}[htbp]
\caption{Few-Shot Pose estimation errors on the Shapenet Chairs dataset.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc}
\toprule
\textbf{Method} & \textbf{Inference} &\multicolumn{2}{c}{\textbf{Pose Estimation errors}}\\
\cmidrule{3-4} 
 & &  \textbf{\textit{Rotation}}& \textbf{\textit{Translation}}  \\
\midrule
\textbf{i-NeRF} & 2-shot samples & 79.31 & 2.03 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (fixed, 24) & 33.52 & 0.11 \\
\textbf{i-$\sigma$SRN (ours)} & multiple (neighbor, 4) &  13.03 & 0.08 \\
\bottomrule
\end{tabular}
}
\label{tab:few-shot-chairs}
\end{table}
